Enabling hand gesture customization on wrist-worn devices

We present a framework for gesture customization requiring minimal examples from users, all without degrading the performance of existing gesture sets. To achieve this, we first deployed a large-scale study (N=500+) to collect data and train an accelerometer-gyroscope recognition model with a cross-user accuracy of 95.7% and a false-positive rate of 0.6 per hour when tested on everyday non-gesture data. Next, we design a few-shot learning framework which derives a lightweight model from our pre-trained model, enabling knowledge transfer without performance degradation. We validate our approach through a user study (N=20) examining on-device customization from 12 new gestures, resulting in an average accuracy of 55.3%, 83.1%, and 87.2% on using one, three, or five shots when adding a new gesture, while maintaining the same recognition accuracy and false-positive rate from the pre-existing gesture set. We further evaluate the usability of our real-time implementation with a user experience study (N=20). Our results highlight the effectiveness, learnability, and usability of our customization framework. Our approach paves the way for a future where users are no longer bound to pre-existing gestures, freeing them to creatively introduce new gestures tailored to their preferences and abilities.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> Summary_of_Changes.tex <==
We thank reviewers for their detailed, insightful, and helpful comments on the paper. We summary the list of changes with the order of the paper sections:

- Significantly trim the abstract (Abs)
- Clarified the difference between the core gestures and the new gestures (Sec 1, 5.1, 5.2, 7.1), add clarified the results for new gestures (Sec 5.2)
- Clarified the reason for collecting high-frequency data and down-sampling (Sec 3.1.1)
- Added more details on the study recruitment (Sec 3.1.1)
- Added more details about the data size of data augmentation and data synthesis (Sec 4.2.3)
- Added more details about the user study instruction (Sec 5.1.3)
- Added more explanation of the increasing false positive rate (Sec 5.2.1)
- Significantly revised the result section of the usability study (Sec 6.3). Added more results description of the similar gesture check (Sec 6.3.1) and NASA results (Sec 6.3.2)
- Added more discussion on the challenges of extending the gesture set (Sec 7.1)
- Added more explanation to Figure 9
- Move the old Table 2 and Fig 11 to the appendix.
- Fixed capitalization in figure and table captions.
- Did a proofreading

==> tex_tab_fig/fig_fewshots_1_or_2gestures.tex <==
\begin{figure}[b]
  \centering
  \begin{subfigure}[b]{.45\columnwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figures/single_gesture_performance.png}
    \vspace{0.15cm}
    \caption{F1 Scores and False Positive of each gesture.}
    \label{subfig:fewshots_results_1_2_gestures:one}
  \end{subfigure}
  \quad
  \begin{subfigure}[b]{.48\columnwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figures/two_gestures_performance.png}
    \caption{\review{F1 Scores between two gestures when both are added as the new gesture set.}}
    \label{subfig:fewshots_results_1_2_gestures:two}
  \end{subfigure}
  \caption{\review{The Prediction Performance when Adding (a) One Gesture, and (b) Two Gestures. All results are based on three shots from each gesture. In (a), higher F1 score indicates better recognition performance. In (b), higher F1 score indicates less confusion between the two newly added gestures.}}
  \label{fig:fewshots_results_1_2_gestures}
  \Description{
Results evaluation of specific gestures.
(a) Barplot of the performance of every single gesture. The Y-axis is the same as the plots in Fig 8. The X-axis shows the 12 gestures ranked by their F1 scores, with the highest on the left, and the lowest on the right. The gestures from the left to right are: Flex, RotateOut, DeviateOut, Spread, RotateIn, DoubleSpread, DeviateIn, Extend, DoublePinkyPinch, PinkyPinch, Peace, and Slide.
(b) A 12 by 12 F1 score matrix when every pair of two gestures are added as new gestures. The column and the raw order is the same as Fig 9.a. Overall, most pair of gestures have high F1 scores. The last three gestures PinkyPinch, Peace, and Slide have relatively lower scores around 75\%.
  }
\end{figure}

==> tex_tab_fig/fig_fewshots_1_or_2gestures_n1.tex <==
\begin{figure}[b]
  \centering
    \centering
    \includegraphics[width=1\columnwidth]{figures/single_gesture_performance.png}
    \caption{Model Performance When Adding One Gesture}
    \label{subfig:fewshots_results_1_2_gestures:one}
\end{figure}

\begin{figure}[b]
    \centering
    \includegraphics[width=1\columnwidth]{figures/two_gestures_performance.png}
    \caption{\review{F1 Scores between Two Gestures When Adding Both Gestures. Higher F1 score indicates less confusion between the two newly added gestures.}}
    \label{subfig:fewshots_results_1_2_gestures:two}
\end{figure}

%   \caption{\review{The Prediction Performance when Adding (a) One Gesture, and (b) Two Gestures. All results are based on three shots from each gesture. In (a), higher F1 score indicates better recognition performance of the gesture. In (b), higher F1 score indicates less confusion between the two newly added gestures.}}
%   \label{fig:fewshots_results_1_2_gestures}
%   \Description{
% Results evaluation of specific gestures.
% (a) Barplot of the performance of every single gesture. The Y-axis is the same as the plots in Fig 8. The X-axis shows the 12 gestures ranked by their F1 scores, with the highest on the left, and the lowest on the right. The gestures from the left to right are: Flex, RotateOut, DeviateOut, Spread, RotateIn, DoubleSpread, DeviateIn, Extend, DoublePinkyPinch, PinkyPinch, Peace, and Slide.
% (b) A 12 by 12 F1 score matrix when every pair of two gestures are added as new gestures. The column and the raw order is the same as Fig 9.a. Overall, most pair of gestures have high F1 scores. The last three gestures PinkyPinch, Peace, and Slide have relatively lower scores around 75\%.
%   }
% \end{figure*}

==> tex_tab_fig/fig_fewshots_1_or_2gestures_old.tex <==
\begin{figure*}[b]
  \centering
  \begin{subfigure}[b]{.45\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/single_gesture_performance.png}
    \vspace{0.2cm}
    \caption{F1 Scores and False Positive of each gesture.}
    \label{subfig:fewshots_results_1_2_gestures:one}
  \end{subfigure}
  \quad \quad
  \begin{subfigure}[b]{.48\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{figures/two_gestures_performance.png}
    \caption{\review{F1 Scores between two gestures when these two gestures are added as the new gesture set.}}
    \label{subfig:fewshots_results_1_2_gestures:two}
  \end{subfigure}
  \caption{\review{The Prediction Performance when Adding (a) One Gesture, and (b) Two Gestures. All results are based on three shots from each gesture. In (a), higher F1 score indicates better recognition performance of the gesture. In (b), higher F1 score indicates less confusion between the two newly added gestures.}}
  \label{fig:fewshots_results_1_2_gestures}
  \Description{
Results evaluation of specific gestures.
(a) Barplot of the performance of every single gesture. The Y-axis is the same as the plots in Fig 8. The X-axis shows the 12 gestures ranked by their F1 scores, with the highest on the left, and the lowest on the right. The gestures from the left to right are: Flex, RotateOut, DeviateOut, Spread, RotateIn, DoubleSpread, DeviateIn, Extend, DoublePinkyPinch, PinkyPinch, Peace, and Slide.
(b) A 12 by 12 F1 score matrix when every pair of two gestures are added as new gestures. The column and the raw order is the same as Fig 9.a. Overall, most pair of gestures have high F1 scores. The last three gestures PinkyPinch, Peace, and Slide have relatively lower scores around 75\%.
  }
\end{figure*}

==> tex_tab_fig/fig_sample.tex <==
\begin{figure*}[b]
\begin{minipage}{0.3\textwidth}
  \centering
  \begin{subfigure}[b]{.49\columnwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figures/gesture_shift.png}
    \caption{Shift}
    \label{subfig:gesture_design:shift}
  \end{subfigure}
%   \quad
  \begin{subfigure}[b]{.49\columnwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figures/gesture_rotate.png}
    \caption{Rotate}
    \label{subfig:gesture_design:rotate}
  \end{subfigure}
  \caption{Waist Gestures}
  \Description{Two humans performing waist gestures. The human on the left is shifting their waist their left side, with the body facing forward. The human on the right is rotating around their torso in their clockwise direction.}
  \label{fig:waist_gesture_design}
\end{minipage} 
\begin{minipage}{0.69\textwidth}
  \centering
  \begin{subfigure}[b]{.49\columnwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figures/topview_study_shift.png}
    \caption{Shift}
    \label{subfig:top_view:shift}
  \end{subfigure}
%   \quad
  \begin{subfigure}[b]{.49\columnwidth}
    \centering
    \includegraphics[width=1\columnwidth]{figures/topview_study_rotate.png}
    \caption{Rotate}
    \label{subfig:top_view:rotate}
  \end{subfigure}
  \caption{Top View of Waist Gestures}
  \Description{Two top views figure to indicate the waist movement and the study setup in Study 1. The figure on the left is for waist shifting gesture. There is a large circle indicating a user's waist maximum shifting range. And there is a small circle with the same center as the large circle, marking out the shift threshold and the region within the small circle is the neutral area. The two circles are equally divided into eight pieces with a dotted line, which indicate regions for the target selection task in Study 1. The figure shows that the user is moving their waist center from the neutral area to the rightmost region, which is the target area.
Similarly, the figure on the right is for waist rotating gesture. Instead of a large circle and a small circle, this time the maximum rotating range and rotating neutral area are represented by a sector of 170 degrees and a small sector of 10 degrees. The small sector sits at the center of the large sector, and represents the direction with the user's forward direction. The large sector was equally divided into four regions. The figure shows that the user is rotating their waist from the neutral area to the right-most region.}
  \label{fig:top_view}
\end{minipage}
\end{figure*}

==> tex_tab_fig/tab_sample1.tex <==
% \begin{table}[t]
% \centering
% % \begin{minipage}[c]{0.63\textwidth}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{cllll}
% \specialrule{1pt}{1pt}{1pt}
% \hline
% \multirow{2}{*}{\makecell{Mea-\\sures}} & \multicolumn{2}{c}{Shifting \& Full Feedback} & \multicolumn{2}{c}{Shifting \& No Feedback} \\ \cline{2-5}
% & \makecell{AOV ($\chi^2(2)$)} & \makecell{Post Hoc} & \makecell{AOV ($\chi^2(2)$)} & \makecell{Post Hoc}  \\
% \hline
% \textit{Success} & $2.42, p = 0.290$ & $\textit{Quick Return}\sim Click\sim Dwell$ & $2.74, p = 0.25$ &  $\textit{Quick Return}\sim Click\sim Dwell$ \\
% \textit{Time} & $34.81, p < 0.001^{***}$  & $\textit{Quick Return}<Click\sim Dwell$    & $5735, p < 0.001^{***}$ & $\textit{Quick Return}<Click<Dwell$ \\
% \textit{NC} & $28.44, p < 0.001^{***}$ & $\textit{Quick Return}<Click\lessapprox Dwell$   & $42.83, p < 0.001^{***}$ & $Click<\textit{Quick Return}<Dwell$  \\
% \hline
% \multirow{2}{*}{\makecell{Mea-\\sures}} & \multicolumn{2}{c}{Rotating \& Full Feedback} & \multicolumn{2}{c}{Rotating \& No Feedback} \\ \cline{2-5}
% & \makecell{AOV ($\chi^2(2)$)} & \makecell{Post Hoc} & \makecell{AOV ($\chi^2(2)$)} & \makecell{Post Hoc}\\
% \hline
% \textit{Success} & $9.71, p = 0.007^{**}$ & $Click\sim \textit{Quick Return} > Dwell$ & $0.82, p = 0.662$ & $\textit{Quick Return}\sim Dwell\sim Click$ \\
% \textit{Time} & $23.05, p < 0.001^{***}$ & $\textit{Quick Return}<Click<Dwell$    & $13.69, p = 0.001^{**}$ & $\textit{Quick Return} \lessapprox Dwell \lessapprox Click$ \\
% \textit{NC} & $3.66, p = 0.161$ & $\textit{Quick Return}\sim Click\sim Dwell$  & $7.76, p = 0.02^{*}$ & $\textit{Quick Return}\sim Click<Dwell$  \\
% \hline
% \specialrule{1pt}{1pt}{1pt}
% \multicolumn{5}{l}{\footnotesize{$^*<0.05$, $^{**}<0.01$, $^{***}<0.001$}, $<$/$>$ implies post hoc significance ($p<0.05$). $\sim$ means no significant difference.}
% \end{tabular}
% }
% % \end{minipage}
% % \hfill
% % \begin{minipage}[c]{0.36\textwidth}
% \caption{Statistical analysis of confirmation techniques.
% \textit{Success}: Success Rate, \textit{Time}: Completion Time,  \textit{NC}: Number of Crossing.
% The relative positions of the selection method in post hoc columns indicate the mean value order.
% % $<$/$>$ implies significance ($p<0.05$). $\lessapprox$/$\gtrapprox$ indicates marginal significance ($p<0.10$). $\sim$ means no significant difference. The same in Table~\ref{tab:study1_results_regionnum}.
% }
% \label{tab:study1_results_confirmation}
% % \end{minipage}
% \end{table}

\begin{table*}[b]
\centering
% \begin{minipage}[c]{0.63\textwidth}
\resizebox{\textwidth}{!}{
\begin{tabular}{cllll}
\specialrule{1pt}{1pt}{1pt}
\hline
\multirow{2}{*}{\makecell{Mea-\\sures}} & \multicolumn{2}{c}{Shifting \& Full Feedback} & \multicolumn{2}{c}{Shifting \& No Feedback} \\ \cline{2-5}
& \makecell{AOV ($\chi^2(2)$)} & \makecell{Post Hoc} & \makecell{AOV ($\chi^2(2)$)} & \makecell{Post Hoc}  \\
\hline
\textit{Success} & $2.42, p = 0.290$ & $\textit{Quick Return}\sim Click\sim Dwell$ & $2.74, p = 0.25$ &  $\textit{Quick Return}\sim Click\sim Dwell$ \\
\textit{Time} & $34.81, p < 0.001^{***}$  & $\textit{Quick Return}<Click\sim Dwell$    & $5735, p < 0.001^{***}$ & $\textit{Quick Return}<Click<Dwell$ \\
\textit{NC} & $28.44, p < 0.001^{***}$ & $\textit{Quick Return}<Click\sim Dwell$   & $42.83, p < 0.001^{***}$ & $Click<\textit{Quick Return}<Dwell$  \\
\hline
\multirow{2}{*}{\makecell{Mea-\\sures}} & \multicolumn{2}{c}{Rotating \& Full Feedback} & \multicolumn{2}{c}{Rotating \& No Feedback} \\ \cline{2-5}
& \makecell{AOV ($\chi^2(2)$)} & \makecell{Post Hoc} & \makecell{AOV ($\chi^2(2)$)} & \makecell{Post Hoc}\\
\hline
\textit{Success} & $9.71, p = 0.007^{**}$ & $Click\sim \textit{Quick Return} > Dwell$ & $0.82, p = 0.662$ & $\textit{Quick Return}\sim Dwell\sim Click$ \\
\textit{Time} & $23.05, p < 0.001^{***}$ & $\textit{Quick Return}<Click<Dwell$    & $13.69, p = 0.001^{**}$ & $\textit{Quick Return} \sim Dwell \sim Click$ \\
\textit{NC} & $3.66, p = 0.161$ & $\textit{Quick Return}\sim Click\sim Dwell$  & $7.76, p = 0.02^{*}$ & $\textit{Quick Return}\sim Click<Dwell$  \\
\hline
\specialrule{1pt}{1pt}{1pt}
\multicolumn{5}{l}{\footnotesize{$^*<0.05$, $^{**}<0.01$, $^{***}<0.001$}, $<$/$>$ implies post hoc significance ($p<0.05$). $\sim$ means no significant difference. Same in Table~\ref{tab:study1_results_regionnum}}
\end{tabular}
}
% \end{minipage}
% \hfill
% \begin{minipage}[c]{0.36\textwidth}
\caption{Statistical analysis of confirmation techniques.
\textit{Success}: Success Rate, \textit{Time}: Completion Time,  \textit{NC}: Number of Crossing.
The relative positions of the selection method in post hoc columns indicate the mean value order. The more favorable techniques (higher \textit{Success}, lower \textit{Time} and \textit{NC}) are put before the less favorable ones.
% $<$/$>$ implies significance ($p<0.05$). $\lessapprox$/$\gtrapprox$ indicates marginal significance ($p<0.10$). $\sim$ means no significant difference. The same in Table~\ref{tab:study1_results_regionnum}.
}
\label{tab:study1_results_confirmation}
\Description{The table can be divided into four parts: shifting with full visual feedback, shifting with no visual feedback, rotating with full visual feedback, and rotating with no visual feedback. In each part, there is the analysis of variance results for success rate, time, and the number of crossings. Three confirmation techniques are compared: quick return, button click, and dwell. Quick return outperforms the other two methods in most cases.}
% \end{minipage}
\end{table*}

==> tex_tab_fig/tab_sample2.tex <==
% \begin{table}[!t]
% \centering
% % \resizebox{1\columnwidth}{!}{
% \begin{tabular}{cccc}
% \specialrule{1pt}{1pt}{1pt}
% \hline
% Task & Operation  &  Waist Gesture & Baseline \\
% \hline
% Music  &  Play/Pause   & Rotate L/R  & Virtual Button Click\\
% Music  &  Vol Up       & Shift FL/FR & Physical Button Click\\
% Music  &  Vol Down     & Shift BL/BR & Physical Button Click\\
% Music  &  Next         & Shift R     & Virtual Button Click\\
% Music  &  Previous     & Shift L     & Virtual Button Click\\
% Call   &  Answer       & Shift R/FR/BR  & Virtual Button Click\\
% Call   &  Reject       & Shift L/FL/BL   & Virtual Button Click\\
% Call   &  Mute         & Rotate L/R  & Physical Button Click\\
% VR     & Slide Left    & Shift L     & TrackPad Click\\
% VR     & Slide Right   & Shift R     & TrackPad Click\\
% VR     & Jump          & Shift FL/FR     & TrackPad Click\\
% VR     & Squat         & Shift BL/BR     & TrackPad Click\\
% VR     & Destroy       & Rotate L/R     & Trigger Click\\
% \hline
% \specialrule{1pt}{1pt}{1pt}
% \end{tabular}
% % }
% \caption{The design of the mapping of \projectname{} gestures and baseline operations for the applications evaluated in the user study.}
% \label{tab:study2_gesture_mapping}
% \end{table}
